A Collaborative Framework for In-network Video Caching in Mobile Networks

Due to explosive growth of online video content in mobile wireless networks, in-network caching is becoming increasingly important to improve the end-user experience and reduce the Internet access cost for mobile network operators. However, caching is a difficult problem due to the very large number of online videos and video requests,limited capacity of caching nodes, and limited bandwidth of in-network links. Existing solutions that rely on static configurations and average request arrival rates are insufficient to handle dynamic request patterns effectively. In this paper, we propose a dynamic collaborative video caching framework to be deployed in mobile networks. We decompose the caching problem into a content placement subproblem and a source-selection subproblem. We then develop SRS (System capacity Reservation Strategy) to solve the content placement subproblem, and LinkShare, an adaptive traffic-aware algorithm to solve the source selection subproblem. Our framework supports congestion avoidance and allows merging multiple requests for the same video into one request. We carry extensive simulations to validate the proposed schemes. Simulation results show that our SRS algorithm achieves performance within 1-3% of the optimal values and LinkShare significantly outperforms existing solutions.

==> Makefile <==
filename=main

all: $(filename).pdf 

$(filename).pdf:$(filename).tex  main.tex  formulation.tex solution.tex \
smhpp.tex  appendix.tex evaluation.tex
	latex $(filename)
	bibtex $(filename)
	latex $(filename)
	latex $(filename)
	dvips $(filename).dvi -o $(filename).ps
	ps2pdf14 -dEmbedAllFonts=true -dPDFSETTINGS=/prepress $(filename).ps $(filename).pdf

pdf: $(filename).ps 
	ps2pdf14 -dEmbedAllFonts=true -dPDFSETTINGS=/prepress $(filename).ps $(filename).pdf

clean:
	rm *.pdf *.ps *.dvi *.bbl  *.blg *.log *.aux 


==> deleted.tex <==

   % The delivery cost originally expressed as $p^k_{ji}$ in
   % (\ref{equal:newd}), requires the full knowledge of the links.
    
   % In practice,
   % depending on the information that serving nodes can access, we outline two
   % basic approaches: e2e information model (E2E Info) and link-state
   % model(LinkInfo).
% For ML, the actual latency for a request is the maximum latency among all scheduled sources.
% This strategy encourages videos to be divided among paths, thus it can avoid the tragedy of common to some extent. In addition, extra balancing methods can be implemented in the division and source selection for requests.
% 
%    Suppose that the load on each link is periodically accessible to each node by router-reporting or measuring over a time slice of $\hbar$. During the time slice, each node $i$ maintains a current flow table for each link locally and separately in order to make proper in-node coordination. The local flow values are updated either after a new local request is scheduled or when global reports or measurements come.
\begin{comment}
\subsubsection{E2E Info Model}\label{ssubsection:ei}
%   

% However, the reality is that in most systems, rather than stringent requirement of full information over all links,
In this model, serving nodes know nothing about the topology of the system as well as the instant information of the links. The end-to-end cost information is more accessible to the serving nodes via e2e info\cite{roughgarden2002bad} or network probing. For example, node $i$ needs the cost for fetching one unit data from node $j$. If there is data flow from $j$ to $i$, such cost is available for $i$ via lower layer protocols, e.g., TCP. Otherwise, node $i$ can use a costless frame to probe it, e.g., a Ping command. We now denote $c^j_{i}$ as the instant end-to-end cost for delivering one unit data from node $j$ to node $i$ which is considered to be stable for the current slot. Thus, for each request at node $i$, we want to solve the following problem 
  
   \begin{sequation}\label{equal:mdtpdistr}
    \min\ \sum_{k\in R_i}\sum_{j\in T_k} x^k_{ji}r_kc^j_i
   \end{sequation}
   subject to
   \begin{sequation}\label{equal:reachmdtp3}
   \forall k\in R_i, \sum_{j\in T_k}x^k_{ji} =1
   \end{sequation}
   and (\ref{equal:xr}).
  Further decomposing the problem (\ref{equal:mdtpdistr}), for each collaborative video request at node $i$, i.e. $ k\in R_i$, we solve the problem below
  \begin{sequation}\label{equal:mdtpdistrrequest}
    \min\ \sum_{j\in T_k} x^k_{ji}r_kc^j_i
   \end{sequation}
   subject to
   \begin{sequation}\label{equal:reachmdtp2}
     \sum_{j\in T_k}x^k_{ji} =1
   \end{sequation}
   and (\ref{equal:xr}).
   
  Apparently, the problem (\ref{equal:mdtpdistrrequest}) can be easily solved analytically with each request is selfishly choosing to the ``nearest'' source in the current slot. This model puts little overhead and requirement over the system, thus can be easily implemented. However, using this model, no coordination is done even within the same node. We omit the description of the algorithm here.

\subsubsection{Link-State Model}\label{ssubsection:link}
    
   In link-state model, the topology of the system and the properties of links are visible to the serving nodes.
\end{comment}


